A Comprehensive Survey on Self-Interpretable Neural Networks

Neural networks have achieved remarkable success across various fields. However, the lack of interpretability limits their practical use, particularly in critical decision-making scenarios. Post-hoc interpretability, which provides explanations for pre-trained models, is often at risk of robustness and fidelity. This has inspired a rising interest in self-interpretable neural networks, which inherently reveal the prediction rationale through the model structures. Although there exist surveys on post-hoc interpretability, a comprehensive and systematic survey of self-interpretable neural networks is still missing. To address this gap, we first collect and review existing works on self-interpretable neural networks and provide a structured summary of their methodologies from five key perspectives: attribution-based, function-based, concept-based, prototype-based, and rule-based self-interpretation. We also present concrete, visualized examples of model explanations and discuss their applicability across diverse scenarios, including image, text, graph data, and deep reinforcement learning. Additionally, we summarize existing evaluation metrics for self-interpretability and identify open challenges in this field, offering insights for future research. To support ongoing developments, we present a publicly accessible resource to track advancements in this domain: https://github.com/yangji721/Awesome-Self-Interpretable-Neural-Network.

==> content/author_bio.tex <==

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figures/people/jiyang.jpg}}]{Yang Ji}
    received the BS degree from Huazhong University of Science and Technology, and the MPhil degree from Hong Kong Baptist University, Department of Computer Science. He is currently working toward the PhD degree with the AI Thrust, The Hong Kong University of Science and Technology (Guangzhou). His research interests include explainable AI, data mining, and intelligent business systems.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figures/people/Ying.jpg}}]{Ying Sun}
    is currently an assistant professor at the Hong Kong University of Science and Technology (Guangzhou). She received the Ph.D. degree in 2022 from the Institute of Computing Technology, Chinese Academy of Sciences, China. Prior to that, she received the B.E. degree in 2017 from Beijing Institute of Technology, China. Her general research interests include Explainable Artificial Intelligence and cross-disciplinary data mining. She has published prolifically in prestigious refereed journals and top-tier conference proceedings such as Nature Communications, Nature Cities, IEEE Transactions on Knowledge and Data Engineering (TKDE), ACM Transactions on Information Systems (TOIS), ACM Transactions on Intelligent Systems and Technology (TIST), SIGKDD, NeurIPS, SIGIR, TheWebConf, IEEE ICDM, etc. She serves as program committee members in numerous top conferences such as KDD, ICML, NeurIPS, IJCAI and AAAI. She has received honors including the CCF Doctoral Dissertation Incentive Award, the Zhu Li Yuehua Outstanding Award, and recognition as a candidate for the ICDM Young Female Scholar Award.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figures/people/yuting.png}}]{Yuting Zhang}
    received the BS degree from Beihang University in 2021, and the MS degree from the Institute of Computing Technology, Chinese Academy of Sciences in 2024. She is currently working toward the PhD degree with The Hong Kong University of Science and Technology (Guangzhou). Her research interests include data mining and recommendation systems. She has published several papers in top-tier conferences and journals, including KDD, MM, ACM Transactions on Information Systems (TOIS).
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figures/people/gaoyuan.jpg}}]{Zhigaoyuan Wang}
    received his B.S. degree from the School of Computer Science and Technology at Beijing University of Posts and Telecommunications. He is currently working toward the PhD degree with the AI thrust, Hong Kong University of Science and Technology (Guangzhou). His research interests include spatiotemporal data mining and AI for science.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figures/people/yuanxin.jpg}}]{Yuanxin Zhuang}
    received the BS degree from China University of Mining and Technology (Beijing), and the MS degree from Beijing University of Posts and Telecommunications. She is currently working toward the PhD degree with the AI Thrust, The Hong Kong University of Science and Technology (Guangzhou). Her research interests include interpretable graph generation and diffusion models.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figures/people/gongzheng.jpg}}]{Zheng Gong}
    received the BS and MS degrees from the school of Computer Science and Technology, University of Science and Technology of China. He is currently working toward the PhD degree with the AI thrust, Hong Kong University of Science and Technology (Guangzhou). His research interests include data mining, graph neural networks and large language models.
\end{IEEEbiography}


\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figures/people/dazhongshen.jpg}}]{Dazhong Shen} (Member, IEEE) earned his Ph.D. degree in Computer Science and Technology from the University of Science and Technology of China (USTC), Hefei, China, in 2023. He is presently an associate researcher at College of Computer Science and Technology, Nanjing University of Aeronautics and Astronautics. He has authored more than 20 journal and conference papers in the fields of Generative Model and Natural Language Processing, including the ACM Transactions on Information Systems (TOIS), IEEE Transactions on Neural Networks and Learning Systems (TNNLS), IEEE Transactions on Knowledge and Data Engineering (TKDE), NeurIPS, SIGKDD, IJCAI, WWW, etc.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figures/people/chuanqin.jpg}}]{Chuan Qin} (Member, IEEE) received the Ph.D. degree in computer science and technology from the University of Science and Technology of China (USTC), Hefei, China, in 2021. He is currently an associate professor at the Computer Network Information Center, Chinese Academy of Sciences. He has authored more than 50 journals and conference papers in the fields of natural language processing and recommender systems, including  IEEE TKDE, IEEE TCSS, ACM TOIS, SIGKDD, SIGIR, WWW, ICDE, NeurIPS, AAAI, IJCAI, and ICDM. He has been honored with the Excellent Award from the President of the Chinese Academy of Sciences (2021), a nomination for the Baidu Scholarship (top 20 globally) (2021), and the Best Student Paper Award of SIGKDD-2018.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figures/people/zhuhengshu.jpg}}]{Hengshu Zhu} (Senior Member, IEEE) is currently a full professor at the Computer Network Information Center (CNIC), Chinese Academy of Sciences (CAS). He received the Ph.D. degree in 2014 and B.E. degree in 2009, both in Computer Science from University of Science and Technology of China (USTC), China. His general area of research is data mining and machine learning, with a focus on developing advanced data analysis techniques for innovative scientific and business applications. He has filed over 100 patents and published more than 180 research papers in top-tier journals (e.g., Nature Cities, Nature Communications, IEEE TKDE, IEEE TMC, ACM TKDD, ACM TOIS) and leading conference proceedings (e.g., KDD, SIGIR, WWW, IJCAI, AAAI). He served as the industry chair of PRICAI-2022, the area chair of SIGKDD, AAAI and IJCAI, and regularly as the (senior) program committee members in numerous top conferences. He was the recipient of the Distinguished Dissertation Award of CAS (2016), the Distinguished Dissertation Award of CAAI (2016), the Special Prize of President Scholarship for Postgraduate Students of CAS (2014), the Best Student Paper Award of KSEM-2011, WAIM-2013, CCDM-2014, and the Best Paper Nomination of ICDM-2014 and WSDM-2022. He is a distinguished member of CCF, and a senior member of ACM, CAAI and IEEE.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figures/people/huixiong.jpg}}]{Hui Xiong} (Fellow, IEEE) is a Chair Professor and Associate Vice-President for Knowledge Transfer at the Hong Kong University of Science and Technology (Guangzhou) and the Founding Head of the Artificial Intelligence Thrust. Previously, he was a Distinguished Professor at Rutgers University. He has published over 400 papers in data science and artificial intelligence, with over 49,000 Google Citations and an h-index of 96. His accolades include the 2021 AAAI Best Paper Award and fellowships from the AAAS, ACM, and IEEE for his contributions to data mining and mobile computing. Dr. Xiong currently serves as the ACM SIGKDD Secretary, Co-Editor-in-Chief of the Encyclopedia of GIS, and Editor-in-Chief of Nature npj | Artificial Intelligence. He has held significant roles in organizing major conferences, including as Program Co-Chair for the ACM SIGKDD and IEEE ICDM. Moreover, he served as the Deputy Dean at Baidu Research, where he played a crucial role in guiding the operations and strategic direction of five research laboratories. Additionally, he has supervised nearly 30 Ph.D. students, many of whom have secured faculty positions at prestigious universities worldwide, including the University of Arizona, Stony Brook University, and the University of Tennessee-Knoxville.
\end{IEEEbiography}

